HM-NAS: Efficient Neural Architecture Search via Hierarchical Masking

The use of automatic methods, often referred to as Neural Architecture Search (NAS), in designing neural network architectures has recently drawn considerable attention. In this work, we present an efficient NAS approach, named HM- NAS, that generalizes existing weight sharing based NAS approaches. Existing weight sharing based NAS approaches still adopt hand-designed heuristics to generate architecture candidates. As a consequence, the space of architecture candidates is constrained in a subset of all possible architectures, making the architecture search results sub-optimal. HM-NAS addresses this limitation via two innovations. First, HM-NAS incorporates a multi-level architecture encoding scheme to enable searching for more flexible network architectures. Second, it discards the hand-designed heuristics and incorporates a hierarchical masking scheme that automatically learns and determines the optimal architecture. Compared to state-of-the-art weight sharing based approaches, HM-NAS is able to achieve better architecture search performance and competitive model evaluation accuracy. Without the constraint imposed by the hand-designed heuristics, our searched networks contain more flexible and meaningful architectures that existing weight sharing based NAS approaches are not able to discover.

==> discussion.tex <==
%!TEX root = neurips_2019.tex

\section{Discussions}
\label{sec.discussion}

\begin{itemize}
    \item How to demonstrate the superiority of our overparameterized network: 1) randomly sampled architectures (simplest search scheme) based on our overparameterized network already perform well, which we attribute to the representation power of our architecture spaces. 2) random search over a few epochs already achieves very competitive results on both datasets, which is remarkable considering it took much less time. 
    
    \item Why overparameterized network is a good init: in contrast to DARTS that only keep the learned cell architecture without its parameter values, our scheme not only offers a good initial point in the search space with non-trivial parameter values, but also helps to avoid an additional bias introduced by handcrafted initialization routines. In fact, this strategy ensures initial architectures are reasonably well-performing even without any search, as suggested by our random initialization results in Table 1.
    
    \item Figure XXX visualizes the best-performing network architecture learned by our algorithm.
    
\end{itemize}



